First observation of the decays $\bar{B}^0_{(s)}\to D_s^+K^-\pi^+\pi^-$ and $\bar{B}^0_s\to D_{s1}(2536)^+\pi^-$

The first observation of the decays $\bar{B}^0_{s}\to D_s^+K^-\pi^+\pi^-$ and $\bar{B}^0\to D_s^+K^-\pi^+\pi^-$ are reported using an integrated luminosity of 1.0 fb$^{-1}$ recorded by the LHCb experiment. The branching fractions, normalized with respect to $\bar{B}^0_{s}\to D_s^+\pi^-\pi^+\pi^-$ and $\bar{B}^0_{s}\to D_s^+K^-\pi^+\pi^-$, respectively, are measured to be {\br(\bar{B}^0_{s}\to D_s^+K^-\pi^+\pi^-)\over\br(\bar{B}^0_{s}\to D_s^+\pi^-\pi^+\pi^-)} &= (5.2\pm0.5\pm0.3)\times10^{-2}, {\br(\bar{B}^0\to D_s^+K^-\pi^+\pi^-)\over\br(\bar{B}^0_{s}\to D_s^+K^-^\pi^+\pi^-)} &= 0.54\pm0.07\pm0.07, where the first uncertainty is statistical and the second is systematic. The $\bar{B}^0_{s}\to D_s^+K^-\pi^+\pi^-$ decay is of particular interest as it can be used to measure the weak phase $\gamma$. First observation of the $\bar{B}^0_s\to D_{s1}(2536)^+\pi^-, D_{s1}^+\to D_s^+\pi^-\pi^+$ decay is also presented, and its branching fraction relative to $\bar{B}^0_{s}\to D_s^+\pi^-\pi^+\pi^-$ is found to be {\br(\bar{B}^0_s\to D_{s1}(2536)^+\pi^-, D_{s1}^+\to D_s^+\pi^-\pi^+)\over\br(\bar{B}^0_{s}\to D_s^+\pi^-\pi^+\pi^-)} &= (4.0\pm1.0\pm0.4)\times10^{-3}.

==> LHCb_comma_separated_author.tex <==
LHCb collaboration:
R. Aaij, 
C. Abellan Beteta, 
A. Adametz, 
B. Adeva, 
M. Adinolfi, 
C. Adrover, 
A. Affolder, 
Z. Ajaltouni, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
Y. Amhis, 
L. Anderlini, 
J. Anderson, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
A. Artamonov , 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
S. Bachmann, 
J.J. Back, 
C. Baesso, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
A. Bates, 
Th. Bauer, 
A. Bay, 
J. Beddow, 
I. Bediaga, 
S. Belogurov, 
K. Belous, 
I. Belyaev, 
E. Ben-Haim, 
M. Benayoun, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
M.-O. Bettler, 
M. van Beuzekom, 
A. Bien, 
S. Bifani, 
T. Bird, 
A. Bizzeti, 
P.M. Bj\o rnstad, 
T. Blake, 
F. Blanc, 
C. Blanks, 
J. Blouw, 
S. Blusk, 
A. Bobrov, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
A. Borgia, 
T.J.V. Bowcock, 
C. Bozzi, 
T. Brambach, 
J. van den Brand, 
J. Bressieux, 
D. Brett, 
M. Britsch, 
T. Britton, 
N.H. Brook, 
H. Brown, 
A. B\"{u}chler-Germann, 
I. Burducea, 
A. Bursche, 
J. Buytaert, 
S. Cadeddu, 
O. Callot, 
M. Calvi, 
M. Calvo Gomez, 
A. Camboni, 
P. Campana, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
H. Carranza-Mejia, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
M. Cattaneo, 
Ch. Cauet, 
M. Charles, 
Ph. Charpentier, 
P. Chen, 
N. Chiapolini, 
M. Chrzaszcz , 
K. Ciba, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
C. Coca, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
G. Corti, 
B. Couturier, 
G.A. Cowan, 
D. Craik, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
P. David, 
P.N.Y. David, 
I. De Bonis, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
P. De Simone, 
D. Decamp, 
M. Deckenhoff, 
H. Degaudenzi, 
L. Del Buono, 
C. Deplano, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
A. Di Canto, 
J. Dickens, 
H. Dijkstra, 
P. Diniz Batista, 
M. Dogaru, 
F. Domingo Bonal, 
S. Donleavy, 
F. Dordei, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
F. Dupertuis, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
D. van Eijk, 
S. Eisenhardt, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
D. Elsby, 
A. Falabella, 
C. F\"{a}rber, 
G. Fardell, 
C. Farinelli, 
S. Farry, 
V. Fave, 
V. Fernandez Albor, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
C. Fitzpatrick, 
M. Fontana, 
F. Fontanelli, 
R. Forty, 
O. Francisco, 
M. Frank, 
C. Frei, 
M. Frosini, 
S. Furcas, 
A. Gallas Torreira, 
D. Galli, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J-C. Garnier, 
J. Garofoli, 
P. Garosi, 
J. Garra Tico, 
L. Garrido, 
C. Gaspar, 
R. Gauld, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
V. Gibson, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
H. Gordon, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
T. Hampson, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
P.F. Harrison, 
T. Hartmann, 
J. He, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
J.A. Hernando Morata, 
E. van Herwijnen, 
E. Hicks, 
D. Hill, 
M. Hoballah, 
P. Hopchev, 
W. Hulsbergen, 
P. Hunt, 
T. Huse, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
V. Iakovenko, 
P. Ilten, 
J. Imong, 
R. Jacobsson, 
A. Jaeger, 
M. Jahjah Hussein, 
E. Jans, 
F. Jansen, 
P. Jaton, 
B. Jean-Marie, 
F. Jing, 
M. John, 
D. Johnson, 
C.R. Jones, 
B. Jost, 
M. Kaballo, 
S. Kandybei, 
M. Karacson, 
T.M. Karbach, 
I.R. Kenyon, 
U. Kerzel, 
T. Ketel, 
A. Keune, 
B. Khanji, 
Y.M. Kim, 
O. Kochebina, 
V. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Korolev, 
A. Kozlinskiy, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
M. Kucharczyk, 
V. Kudryavtsev, 
T. Kvaratskheliya, 
V.N. La Thi, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
R.W. Lambert, 
E. Lanciotti, 
G. Lanfranchi, 
C. Langenbruch, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
O. Leroy, 
T. Lesiak, 
Y. Li, 
L. Li Gioi, 
M. Liles, 
R. Lindner, 
C. Linn, 
B. Liu, 
G. Liu, 
J. von Loeben, 
J.H. Lopes, 
E. Lopez Asamar, 
N. Lopez-March, 
H. Lu, 
J. Luisier, 
H. Luo, 
A. Mac Raighne, 
F. Machefert, 
I.V. Machikhiliyan, 
F. Maciuc, 
O. Maev, 
J. Magnin, 
M. Maino, 
S. Malde, 
G. Manca, 
G. Mancinelli, 
N. Mangiafave, 
U. Marconi, 
R. M\"{a}rki, 
J. Marks, 
G. Martellotti, 
A. Martens, 
L. Martin, 
A. Mart\'{i}n S\'{a}nchez, 
M. Martinelli, 
D. Martinez Santos, 
D. Martins Tostes, 
A. Massafferri, 
R. Matev, 
Z. Mathe, 
C. Matteuzzi, 
M. Matveev, 
E. Maurice, 
A. Mazurov, 
J. McCarthy, 
G. McGregor, 
R. McNulty, 
M. Meissner, 
M. Merk, 
J. Merkel, 
D.A. Milanes, 
M.-N. Minard, 
J. Molina Rodriguez, 
S. Monteil, 
D. Moran, 
P. Morawski, 
R. Mountain, 
I. Mous, 
F. Muheim, 
K. M\"{u}ller, 
R. Muresan, 
B. Muryn, 
B. Muster, 
J. Mylroie-Smith, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
I. Nasteva, 
M. Needham, 
N. Neufeld, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
M. Nicol, 
V. Niess, 
N. Nikitin, 
T. Nikodem, 
A. Nomerotski, 
A. Novoselov, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Oggero, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
M. Orlandea, 
J.M. Otalora Goicochea, 
P. Owen, 
B.K. Pal, 
A. Palano, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
C. Parkes, 
C.J. Parkinson, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
G.N. Patrick, 
C. Patrignani, 
C. Pavel-Nicorescu, 
A. Pazos Alvarez, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
D.L. Perego, 
E. Perez Trigo, 
A. P\'{e}rez-Calero Yzquierdo, 
P. Perret, 
M. Perrin-Terrin, 
G. Pessina, 
K. Petridis, 
A. Petrolini, 
A. Phan, 
E. Picatoste Olloqui, 
B. Pie Valls, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
S. Playfer, 
M. Plo Casasus, 
F. Polci, 
G. Polok, 
A. Poluektov, 
E. Polycarpo, 
D. Popov, 
B. Popovici, 
C. Potterat, 
A. Powell, 
J. Prisciandaro, 
V. Pugatch, 
A. Puig Navarro, 
W. Qian, 
J.H. Rademacker, 
B. Rakotomiaramanana, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
S. Redford, 
M.M. Reid, 
A.C. dos Reis, 
S. Ricciardi, 
A. Richards, 
K. Rinnert, 
V. Rives Molina, 
D.A. Roa Romero, 
P. Robbe, 
E. Rodrigues, 
P. Rodriguez Perez, 
G.J. Rogers, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. Rouvinet, 
T. Ruf, 
H. Ruiz, 
G. Sabatino, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
C. Salzmann, 
B. Sanmartin Sedes, 
M. Sannino, 
R. Santacesaria, 
C. Santamarina Rios, 
R. Santinelli, 
E. Santovetti, 
M. Sapunov, 
A. Sarti, 
C. Satriano, 
A. Satta, 
M. Savrie, 
P. Schaack, 
M. Schiller, 
H. Schindler, 
S. Schleich, 
M. Schlupp, 
M. Schmelling, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
M. Seco, 
A. Semennikov, 
K. Senderowska, 
I. Sepp, 
N. Serra, 
J. Serrano, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
P. Shatalov, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
O. Shevchenko, 
V. Shevchenko, 
A. Shires, 
R. Silva Coutinho, 
T. Skwarnicki, 
N.A. Smith, 
E. Smith, 
M. Smith, 
K. Sobczak, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
A. Sparkes, 
P. Spradlin, 
F. Stagni, 
S. Stahl, 
O. Steinkamp, 
S. Stoica, 
S. Stone, 
B. Storaci, 
M. Straticiuc, 
U. Straumann, 
V.K. Subbiah, 
S. Swientek, 
M. Szczekowski, 
P. Szczypka, 
T. Szumlak, 
S. T'Jampens, 
M. Teklishyn, 
E. Teodorescu, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
S. Tolk, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
M.T. Tran, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
M. Ubeda Garcia, 
A. Ukleja, 
D. Urner, 
U. Uwer, 
V. Vagnoni, 
G. Valenti, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
I. Videau, 
D. Vieira, 
X. Vilasis-Cardona, 
J. Visniakov, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
H. Voss, 
R. Waldi, 
R. Wallace, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
A.D. Webber, 
D. Websdale, 
M. Whitehead, 
J. Wicht, 
D. Wiedner, 
L. Wiggers, 
G. Wilkinson, 
M.P. Williams, 
M. Williams, 
F.F. Wilson, 
J. Wishahi, 
M. Witek, 
W. Witzeling, 
S.A. Wotton, 
S. Wright, 
S. Wu, 
K. Wyllie, 
Y. Xie, 
F. Xing, 
Z. Xing, 
Z. Yang, 
R. Young, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
F. Zhang, 
L. Zhang, 
W.C. Zhang, 
Y. Zhang, 
A. Zhelezov, 
L. Zhong, 
A. Zvyagin

